Fantastic Copyrighted Beasts and How (Not) to Generate Them

Recent studies show that image and video generation models can be prompted to reproduce copyrighted content from their training data, raising serious legal concerns about copyright infringement. Copyrighted characters (e.g., Mario, Batman) present a significant challenge: at least one lawsuit has already awarded damages based on the generation of such characters. Consequently, commercial services like DALL-E have started deploying interventions. However, little research has systematically examined these problems: (1) Can users easily prompt models to generate copyrighted characters, even if it is unintentional?; (2) How effective are the existing mitigation strategies? To address these questions, we introduce a novel evaluation framework with metrics that assess both the generated image's similarity to copyrighted characters and its consistency with user intent, grounded in a set of popular copyrighted characters from diverse studios and regions. We show that state-of-the-art image and video generation models can still generate characters even if characters' names are not explicitly mentioned, sometimes with only two generic keywords (e.g., prompting with "videogame, plumber" consistently generates Nintendo's Mario character). We also introduce semi-automatic techniques to identify such keywords or descriptions that trigger character generation. Using this framework, we evaluate mitigation strategies, including prompt rewriting and new approaches we propose. Our findings reveal that common methods, such as DALL-E's prompt rewriting, are insufficient alone and require supplementary strategies like negative prompting. Our work provides empirical grounding for discussions on copyright mitigation strategies and offers actionable insights for model deployers implementing these safeguards.

==> tables/main_results.tex <==
\begin{table}[t]
    \caption{Performance of all intervention strategies on the Playground v2.5 model. We run each strategy three times, and report the mean and standard deviation of the number of detected copyrighted characters ($\mathsf{DETECT}$, lower is better) and the consistency with user intent ($\mathsf{CONS}$, higher is better). Including the character's name in the negative prompts is highly important for reducing $\mathsf{DETECT}$. Combining prompt rewriting and negative prompts can effectively reduce $\mathsf{DETECT}$ from 30 to 5, without significantly degrading $\mathsf{CONS}$. \yang{WARNING: This table is subject to major changes; pls skip it for now}
 % \yang{TODO: Explain lower and upper bound numbers for CONS}
 % \peter{What's the difference between keywords and LAION keywords? Maybe say curated keywords?}
 } 
    \small
    % \setlength{\tabcolsep}{6pt}
    \label{tab:results}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcc|ccc}
    \toprule
    \multirow{2}{*}{\bf Negative Prompt} & \multicolumn{2}{c|}{\bf Prompt: Target's name} & \multicolumn{2}{c}{\bf Prompt: Rewritten prompt}\\
       
          & $\mathsf{DETECT}$ ($\downarrow$) &  $\mathsf{CONS}$ ($\uparrow$)  & $\mathsf{DETECT}$ ($\downarrow$) &  $\mathsf{CONS}$ ($\uparrow$)\\
    \midrule
        None & \da{$30.33_{\pm 1.89}$} & $\mathbf{0.75}_{\pm 0.01}$ & $14.33_{\pm 2.62}$ & $0.80_{\pm 0.01}$ \\
        \midrule
        \rowcolor{lightgray} "Copyrighted character" & $30.33_{\pm 1.25}$ & $0.74_{\pm 0.01}$ & $17.33_{\pm 1.70}$ & $0.80_{\pm 0.01}$ \\
        + 1 curated keyword & $30.00_{\pm 0.82}$ & $0.74_{\pm 0.01}$ & $16.00_{\pm 1.63}$ & $0.81_{\pm 0.01}$ \\
        + 5 curated keywords & $26.67_{\pm 0.94}$ & $0.70_{\pm 0.02}$ & $11.33_{\pm 2.05}$ & $\mathbf{0.82}_{\pm 0.00}$\\
        + 10 curated keywords & $26.33_{\pm 1.25}$ & $0.73_{\pm 0.01}$ & $10.67_{\pm 2.49}$ & $\mathbf{0.82}_{\pm 0.00}$\\
        + 5 curated keywords \& 5 keywords from LAION & $\mathbf{25.00}_{\pm 1.89}$ & $0.71_{\pm 0.01}$ & $\mathbf{9.33}_{\pm 1.70}$ & $0.81_{\pm 0.00}$ \\
        \midrule
        \rowcolor{lightgray} Target's name & $23.67_{\pm 2.62}$ & $0.76_{\pm 0.01}$ & $7.67_{\pm 0.47}$ & $0.81_{\pm 0.01}$ \\
        + 1 curated keyword & $23.67_{\pm 2.87}$ & $0.76_{\pm 0.01}$ & $7.67_{\pm 0.47}$ & $\mathbf{0.82}_{\pm 0.01}$ \\
        + 5 curated keywords & $23.33_{\pm 2.05}$ & $0.72_{\pm 0.01}$ & $5.67_{\pm 2.05}$ & $0.81_{\pm 0.01}$ \\
        + 10 curated keywords & $23.00_{\pm 2.45}$ & $0.70_{\pm 0.02}$ & $5.67_{\pm 1.70}$ & $0.81_{\pm 0.01}$ \\
        + 5 curated keywords \& 5 keywords from LAION & $\mathbf{20.33}_{\pm 2.16}$ & $0.70_{\pm 0.02}$ & \da{$\mathbf{5.00}_{\pm 0.82}$} & $\mathbf{0.82}_{\pm 0.01}$ \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/model_summary.tex <==
\begin{table}[t]
    \centering
    \caption{The combination of prompt-rewriting and negative prompts can significantly reduce $\mathsf{DETECT}$ while mostly preserving $\mathsf{CONS}$ across all 5 open-source models tested, making it a promising candidate for copyright-protection intervention. \lucy{Add what the negative prompt is exactly.} \yang{TODO: the second column needs to be updated}} 
    \label{tab:intervention}
    \small
    \setlength{\tabcolsep}{3pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcc|cccc}
    \toprule
        \multirow{2}{*}{\bf Model} & \multicolumn{2}{c|}{\bf  w/o Intervention} & \multicolumn{2}{c}{\bf  w/ Prompt Rewriting \& Negative Prompt}  \\
        &  $\mathsf{DETECT}$ ($\downarrow$) &  $\mathsf{CONS}$ ($\uparrow$) & $\mathsf{DETECT}$ ($\downarrow$) &  $\mathsf{CONS}$ ($\uparrow$)  \\
    \midrule
     Playground v2.5~\citep{li2024playground}     & $30.33_{\pm1.89}$  & $0.75_{\pm0.01}$ & $5.00_{\pm 0.82}$ & $0.82_{\pm0.01}$ \\
      Stable Diffusion XL~\citep{podell2023sdxl} & $33.00_{\pm1.00}$ & $0.73_{\pm 0.01}$ & $2.00_{\pm 1.00}$ & $0.76_{\pm 0.01}$\\
      PixArt-$\alpha$~\citep{chen2023pixart} & $24.67_{\pm0.58}$ &  $0.79_{\pm 0.01}$ & $2.67_{\pm1.15}$ & $0.69_{\pm 0.01}$ \\
       DeepFloyd IF~\citep{deepfloyd2023if} & $33.67_{\pm1.53}$ & $0.71_{\pm 0.01}$ & $1.67_{\pm0.58}$ & $0.74_{\pm 0.02}$\\
    \midrule
       VideoFusion (\citep{VideoFusion})& $28.33_{\pm 1.89}$ & $0.68_{\pm 0.01}$ & $12.00_{\pm 1.41}$ & $0.77_{\pm 0.01}$
\\
    \bottomrule
    \end{tabular}
    }
\end{table}
